Luenberger observers for two-gene regulatory networks with sigmoidal regulation: explicit observability conditioning, polytopic convergence certificates, and a logistic--Hill comparison

Only a few species of a gene regulatory network can be measured, so the others must be reconstructed by a state observer, and how well this works depends on the function chosen to describe regulation. We examine this for the two-gene negative feedback loop with one measured protein, for monotone regulation functions including the logistic function and the Hill function with its leaky and shifted variants. Using standard tools, we show that the answer is set by the smallest and the largest slope of the regulation function on the concentrations visited. For every function considered, the unmeasured concentration can be recovered from the measured signal and its rate of change, with an error sensitivity set by the smallest slope. A Luenberger observer with explicit gains converges exponentially from any initial guess and tolerates bounded measurement noise whenever a checkable matrix condition involving only the largest slope holds, as it does for every model examined with bounded slopes. The guaranteed rate cannot exceed the degradation rate of the unmeasured protein unless the smallest slope is positive, and faster rates then hold only for small initial errors. All reported rates are certified from above and below. At matched threshold and steepness, no family is uniformly better: the logistic function is better conditioned when the threshold lies mid-range, leaky or shifted Hill functions when it lies low. Hill functions with exponent below one have an unbounded slope at zero concentration and lose the global guarantee, which logistic and shifted Hill functions keep.

==> tab_certificates.tex <==
Baseline, global & $0.0999$ & $0.1000$ & Prop.~3 & $6.994$ & $0.2648$ & $0.153$ & $-1.1\times10^{-6}$ & -- \\
Baseline, set, $\rho=0$ & $0.1111$ & $0.1112$ & Prop.~3 & $6.111$ & $0.3235$ & $0.1808$ & $-1.3\times10^{-5}$ & -- \\
Baseline, set, $\rho=1$ & $0.1041$ & $0.1042$ & Prop.~3 & $5.971$ & $0.3141$ & $0.184$ & $-3.6\times10^{-6}$ & -- \\
Baseline, set, $\rho=5$ & $0.1000$ & $0.1001$ & Prop.~3 & $6.9919$ & $0.2647$ & $0.15304$ & $-6.0\times10^{-6}$ & -- \\
\midrule
A: Logistic, set & $0.1119$ & $0.1120$ & Prop.~3 & $5.894$ & $0.3382$ & $0.1891$ & $-2.3\times10^{-5}$ & -- \\
A: Logistic, global & $0.0999$ & $0.1000$ & Prop.~3 & $6.994$ & $0.2648$ & $0.153$ & $-1.1\times10^{-6}$ & -- \\
A: Hill, set & $0.0999$ & $0.1000$ & Prop.~3 & $6.858$ & $0.2714$ & $0.1566$ & $-1.3\times10^{-5}$ & -- \\
A: Hill, global & $0.0999$ & $0.1000$ & Prop.~3 & $6.858$ & $0.2714$ & $0.1566$ & $-1.3\times10^{-5}$ & -- \\
A: Leaky Hill, set & $0.1001$ & $0.1002$ & Prop.~3 & $7.346$ & $0.2761$ & $0.1465$ & $-1.0\times10^{-5}$ & -- \\
A: Leaky Hill, global & $0.0999$ & $0.1000$ & Prop.~3 & $7.35$ & $0.2763$ & $0.1465$ & $-1.6\times10^{-5}$ & -- \\
A: Shifted Hill, set & $0.1001$ & $0.1002$ & dual & $6.895$ & $0.2691$ & $0.1555$ & $-1.1\times10^{-6}$ & $1.4\times10^{-6}$ \\
A: Shifted Hill, global & $0.0999$ & $0.1000$ & Prop.~3 & $6.899$ & $0.2693$ & $0.1555$ & $-1.4\times10^{-5}$ & -- \\
\midrule
B: Logistic, set & $0.0994$ & $0.0995$ & dual & $4.771$ & $0.398$ & $0.2428$ & $-2.1\times10^{-5}$ & $1.1\times10^{-6}$ \\
B: Logistic, global & $0.0994$ & $0.0995$ & dual & $4.771$ & $0.398$ & $0.2428$ & $-2.1\times10^{-5}$ & $1.1\times10^{-6}$ \\
B: Hill, set & $0.0994$ & $0.0995$ & dual & $5.582$ & $0.5498$ & $0.2333$ & $-3.0\times10^{-5}$ & $2.8\times10^{-6}$ \\
B: Hill, global & $0.0994$ & $0.0995$ & dual & $5.582$ & $0.5498$ & $0.2333$ & $-3.0\times10^{-5}$ & $2.8\times10^{-6}$ \\
B: Leaky Hill, set & $0.0999$ & $0.1000$ & dual & $7.11$ & $0.969$ & $0.2727$ & $-5.3\times10^{-6}$ & $8.5\times10^{-8}$ \\
B: Leaky Hill, global & $0.0978$ & $0.0979$ & dual & $7.1183$ & $0.9702$ & $0.27272$ & $-4.5\times10^{-5}$ & $3.8\times10^{-7}$ \\
B: Shifted Hill, set & $0.0999$ & $0.1000$ & dual & $5.333$ & $0.4821$ & $0.2311$ & $-3.7\times10^{-5}$ & $1.5\times10^{-6}$ \\
B: Shifted Hill, global & $0.0995$ & $0.0996$ & dual & $5.336$ & $0.48236$ & $0.23101$ & $-4.6\times10^{-6}$ & $7.4\times10^{-6}$ \\
\midrule
C: Logistic, global & $0.0999$ & $0.1000$ & Prop.~3 & $71.98$ & $0.2679$ & $0.01489$ & $-2.6\times10^{-6}$ & -- \\
C: Logistic, set $[0,10]$ & $0.7794$ & $0.7795$ & Prop.~3 & $166.5$ & $4.092$ & $0.1066$ & $-1.5\times10^{-6}$ & -- \\
C: Hill, set $[1,10]$ & $0.2741$ & $0.2742$ & dual & $30.67$ & $0.8511$ & $0.05622$ & $-2.0\times10^{-6}$ & $2.4\times10^{-7}$ \\
C: Leaky Hill, set $[1,10]$ & $0.2676$ & $0.2677$ & dual & $32.57$ & $0.8111$ & $0.0509$ & $-7.5\times10^{-6}$ & $3.3\times10^{-8}$ \\
C: Shifted Hill, global & $0.0929$ & $0.0930$ & dual & $31.87$ & $0.8843$ & $0.05592$ & $-1.2\times10^{-5}$ & $4.2\times10^{-9}$ \\
C: Shifted Hill, set $[0,10]$ & $0.2698$ & $0.2699$ & dual & $29.01$ & $0.8049$ & $0.0568$ & $-3.1\times10^{-6}$ & $4.6\times10^{-8}$ \\


==> tab_finite_rho.tex <==
Logistic & $[-0.5,10.5]$ & $[0.0232,0.0250]$ & $0.7584$ & $137.6$ & $3.594$ & $0.1011$ & $-1.6\times10^{-6}$ & $0.00722$ & $138.1$ & $0.0036$ \\
Hill & $[0.5,10.5]$ & $[0.0115,0.1825]$ & $0.0911$ & $21.226$ & $0.5883$ & $0.063418$ & $-4.5\times10^{-6}$ & $0.0471$ & $21.2$ & $0.0235$ \\
Leaky Hill & $[0.5,10.5]$ & $[0.0109,0.1734]$ & $0.0738$ & $22.77$ & $0.5665$ & $0.05801$ & $-7.6\times10^{-6}$ & $0.0439$ & $22.8$ & $0.0219$ \\
Shifted Hill & $[-0.5,10.5]$ & $[0.0126,0.1138]$ & $0.2621$ & $29.13$ & $0.8083$ & $0.05675$ & $-9.5\times10^{-6}$ & $0.0343$ & $29.2$ & $0.0171$ \\


==> tab_thresholds.tex <==
Hill & $[0.367,10]$ & infeasible & dual certificate at $\alpha=0$, $\lambda_{\min}(G)=5.2\times10^{-6}$ \\
Hill & $[0.368,10]$ & feasible & $P=\bigl(\begin{smallmatrix}18.478&0.51177\\0.51177&0.068293\end{smallmatrix}\bigr)$, residual $-2.9\times10^{-5}$ at $\alpha=3.2\times10^{-4}$ \\
Leaky Hill & $[0.391,10]$ & infeasible & dual certificate at $\alpha=0$, $\lambda_{\min}(G)=1.9\times10^{-6}$ \\
Leaky Hill & $[0.392,10]$ & feasible & $P=\bigl(\begin{smallmatrix}20.406&0.5074\\0.5074&0.061623\end{smallmatrix}\bigr)$, residual $-5.3\times10^{-5}$ at $\alpha=6.0\times10^{-4}$ \\

